Exploring Quark Matter

These proceedings contain research results presented during the Workshops "Quark Matter in Astro- and Particle Physics" held at the University of Rostock, November 27-29, 2000 and "Dynamical Aspects of the QCD Phase Transition" held at the ECT* in Trento, March 12-15, 2001.

==> SOURCE/dedication.tex <==
\pagestyle{empty}
\hspace*{7cm}

$\left. \right.$

\vspace*{7cm}
\noindent
{\large \bf Dedicated to our academic teacher Gerd R{\"o}pke\\
on the occasion of his 60th birthday.}

\newpage


==> SOURCE/gamzleer2.tex <==
\pagestyle{empty}
\hspace*{7cm}

$\left. \right.$

\newpage

==> SOURCE/leer.tex <==
\hspace*{7cm}

$\left. \right.$

\newpage
